Spectral methods for volatility derivatives

In the first quarter of 2006 Chicago Board Options Exchange (CBOE) introduced, as one of the listed products, options on its implied volatility index (VIX). This created the challenge of developing a pricing framework that can simultaneously handle European options, forward-starts, options on the realized variance and options on the VIX. In this paper we propose a new approach to this problem using spectral methods. We use a regime switching model with jumps and local volatility defined in \cite{FXrev} and calibrate it to the European options on the S&P 500 for a broad range of strikes and maturities. The main idea of this paper is to "lift" (i.e. extend) the generator of the underlying process to keep track of the relevant path information, namely the realized variance. The lifted generator is too large a matrix to be diagonalized numerically. We overcome this difficulty by applying a new semi-analytic algorithm for block-diagonalization. This method enables us to evaluate numerically the joint distribution between the underlying stock price and the realized variance, which in turn gives us a way of pricing consistently European options, general accrued variance payoffs and forward-starting and VIX options.

==> Conclusion.tex <==
In this paper we introduce an approach for pricing 
derivatives that
depend on pure realized variance (such as volatility swaps and variance swaptions)
and derivatives that are sensitive to the implied volatility smile (such
as forward-starting options)
within the same framework. 

The underlying model is a stochastic volatility
model with jumps that has the ability to switch between different CEV
regimes and therefore exhibit different
characteristics in different market scenarios.
The structure of the model allows it to be calibrated to 
the implied volatility surface with minimal explicit time-dependence.
The stationary nature of the model is best described by the implied forward
smile behaviour that can be observed in figures~\ref{fig:fs_skew3m},
\ref{fig:fs_skew6m}, \ref{fig:fs_skew1y} and~\ref{fig:fs_skew2y}.

The model is then extended in such a way that it captures 
the realized variance of the underlying process, while retaining
complete numerical solubility. Two key ideas that make it possible
to keep track of the path information numerically are:
\begin{itemize}
\item the observation that path-dependence can be expressed as the
      lifting of a Markov generator, and that
\item the state-space of the lifted process can be chosen 
      to be on the circle so that 
      numerical tractability is retained.      
\end{itemize}
Having obtained the joint
probability distribution function for the realized variance 
and the underlying process, we outline the pricing algorithms for 
derivatives that are sensitive to the realized variance
and the implied volatility within the same model. 


==> VolDer.tex <==
In this appendix we are going to give a brief description of the volatility
derivatives discussed in this paper. We start with 
the simplest case, namely a forward on the realized variance,
which defines a variance swap. 
In subsection~\ref{subsec:Vol} we define options
with payoffs that are general functions of realized variance. 
Subsection~\ref{subsec:VIX} concerns derivatives
that are dependent on implied volatility. In particular
we recall the definition of the forward-starting options
and of the implied volatility index.

\subsection{Variance swaps}
\label{subsec:Var}
As mentioned above, a variance swap expiring at time
$T$
is simply a forward contract
on the realized variance
$\Sigma_T$,
quoted in annual terms,
of the underlying stock (or index)
over the time interval
$[0,T]$. 
The payoff is therefore of the form
$$(\Sigma_T-K_{\mathrm{var}})N,$$
where 
$K_{\mathrm{var}}$
is the strike and 
$N$
is the notional of the contract. The fair value of
the variance is the delivery price
$K_{\mathrm{var}}$
which makes the swap have zero value at inception.

At present such contracts are liquidly traded for most 
major indices.
The delivery price is usually quoted in the markets 
as the square of the realized volatility, i.e.
$K_{\mathrm{var}}=K^2$
where 
$K$
is a value of realized volatility expressed in percent. The notional
$N$
is usually quoted in dollars per square of the volatility 
point\footnote{A \textit{volatility point}
is one basis point of volatility, i.e. 
$0.01$
if volatility is quoted in percent. This means that the quote
for the notional
value of the variance swap tells us how much the swap owner 
gains if the realized variance increases by 
$0.0001=0.01^2$.}. 

A key part of the specification of a 
variance swap contract is how one measures
the realized variance
$\Sigma_T$.
There are a number of ways in which discretely sampled 
returns of an index (or of an 
index future\footnote{The reason for
considering index futures rather than the index itself
is twofold. The futures are used for hedging
options on the index because they are much easier
to trade than the whole portfolio of stocks 
that the index comprises. 
Also, it is well-known that futures prices are martingales
under the appropriate risk-neutral measure which depends on the
frequency of mark-to-market. If the futures contract 
marks to market continuously, then the price process
$F_t$
is a martingale in the risk-neutral measure induced by the money
market account as a numeraire. Otherwise 
we have to take the rollover strategy, with the same frequency as 
mark-to-market, as our numeraire to obtain the martingale measure
for 
$F_t$.}
$F_t$)
can be calculated and used for
defining the realized variance.
We will now describe the two most common approaches.

The usual definition of the annualized
realized (i.e. accrued) variance of the underlying process
$F_t$
in the period
$[0,T]$,
using logarithmic returns,
is 
$\frac{d}{n}\sum_{i=1}^n(\log\frac{F_{t_i}}{F_{t_{i-1}}})^2,$
where times 
$t_i$,
for 
$i=0,\ldots,n$,
are business days from
now
$t_0=0$
until expiry
$t_n=T$.
The normalization constant 
$d$
is the number of trading days per year.
Another frequently used
definition of the realized variance
is given by
$\frac{d}{n}\sum_{i=1}^n(\frac{F_{t_i}-F_{t_{i-1}}}{F_{t_{i-1}}})^2.$
It is a standard fact 
about continuous square-integrable martingales
that 
in the limit,
as we make partitions of the interval
$[0,T]$
finer and finer,
both sums exhibit the following behaviour\footnote{
Notice also that these equalities hold because the difference
of the process
$\log(F_t)$
and
$\int_0^t\frac{dF_u}{F_u}$
is of finite variation, which is a consequence of
It\^{o}'s lemma (see theorem 3.3 in~\cite{Karatzas}).}: 
$$\langle\log F\rangle_t = \lim_{n\rightarrow \infty}
\sum_{i=1}^n\left(\log\frac{F_{t_i}}{F_{t_{i-1}}} \right)^2 =
\lim_{n\rightarrow \infty}
\sum_{i=1}^n\left(\frac{F_{t_i}-F_{t_{i-1}}}{F_{t_{i-1}}} \right)^2.
$$
The convergence here is in probability and 
the process  
$\langle\log F\rangle_t$
is the quadratic-variation\footnote{For a precise 
definition of a quadratic-variation of continuous 
square-integrable martingales see chapter 1 of~\cite{Karatzas}.} 
process
associated to
$\log(F_t)$.

In our framework the underlying process
$F_t$
is a continuous-time Markov chain (see chapter 6 of~\cite{Norris}
for definitions and basic properties). We define the annualized 
realized variance
$\Sigma_T$
(of 
$F_t$
over the time interval
$[0,T]$)
to be the limit
\begin{eqnarray}
\label{eq:DiscreteVar}
\Sigma_T:=\frac{1}{T}\lim_{\rho(n)\rightarrow 0}
\sum_{i=1}^n\left(\frac{F_{t_i}-F_{t_{i-1}}}{F_{t_{i-1}}} \right)^2,
\end{eqnarray}
where, for every 
$n\in\NN$,
the set
$(t_i)_{i=0,\ldots,n}$
is a strictly increasing sequence of times between 0 and 
$T$
and
$\rho(n):=\max\{t_i-t_{i-1};\>i=1,\ldots,n\}$
is the size of the maximal subinterval 
given by the sequence 
$(t_i)_{i=0,\ldots,n}$
(cf. definitions~(\ref{eq:InstVar}) in section~\ref{sec:path}
and~(\ref{eq:VarGen}), (\ref{eq:InstDrift}) in subsection~\ref{subsec:Lifting}).
It should be noted that the techniques described in 
sections~\ref{sec:path} and~\ref{sec:Bloc},
which provide numerical solubility for our model,
can be generalized to the situation where 
the realized variance is defined 
as a  
discretely sampled sum
in~(\ref{eq:DiscreteVar})
but
without the limit.
We are not going to pursue this line of thought any further, but 
should notice that
the discrete definition of the realized variance
would require 
the application of the block-diagonalization
algorithm (appendix~\ref{sec:Bloc}) to the probability kernel 
between any two consecutive observation times
$t_i$
rather than the 
application of the algorithm to 
the Markov generator directly, which is what 
is done in
section~\ref{sec:pricing}.

\subsection{General payoffs of the realized variance}
\label{subsec:Vol}
A \textit{volatility swap} is a derivative given 
by the payoff 
$$(\sigma^R_T-K_{\mathrm{vol}})N,$$
where 
$\sigma^R_T$
is the realized volatility over the time interval
$[0,T]$
quoted in annual terms, 
$K_{\mathrm{vol}}$
is the annualized volatility strike
and
$N$
is the notional in dollars per volatility point. The market convention
for calculating the annualized realized volatility 
$\sigma^R_T$
differs slightly
from the usual statistical measure\footnote{Given a sample of 
$n$
values
$X_1,\ldots,X_n$
with the mean
$\mu=\frac{1}{n}\sum_{i=1}^nX_i$,
the unbiased statistical estimation of the
standard deviation is given by
$$\sqrt{\frac{1}{n-1}\sum_{i=1}^n\left(X_i-\mu\right)^2}.$$}
of a standard deviation of any discrete sample
and is given by the formula
$$\sigma^R_T=\sqrt{\frac{d}{n}\sum_{i=1}^n
\left(\frac{F_{t_i}-F_{t_{i-1}}}{F_{t_{i-1}}}\right)^2},$$
where 
$d$
is the number of trading days per year and
$t_i$
are business days from
now
$t_0=0$
until expiry
$t_n=T$
of the contract.
For our purposes we shall define realized volatility 
$\sigma^R_T$,
quoted in annual terms,
over the time interval
$[0,T]$
as
$$\sigma^R_T:=\sqrt{\Sigma_T},$$
where
$\Sigma_T$
is the annualized realized variance defined in~(\ref{eq:DiscreteVar}).
It is clear from this definition that the payoff of the 
volatility swap can be
view as a non-linear function of the realized variance.

Since volatility swaps are always entered into at equilibrium,
an important issue is the determination of the fair strike
$K_{\mathrm{vol}}$
for any given maturity
$T$.
As discussed in section~\ref{sec:Intro}, a term structure of
such strikes must be part of the market data that some 
models require
(e.g.~\cite{Buehler}) in order to be calibrated.
In our case the strikes
$K_{\mathrm{vol}}$,
for any maturity, are implied by the model which 
uses as its calibration data 
the market implied vanilla surface.
The value of 
$K_{\mathrm{vol}}$
for a given maturity 
$T$
is then given by the expectation
$\EE_0[\sqrt{\Sigma_T}]$,
which can easily be obtained as soon as we have 
the probability distribution function
for
$\Sigma_T$.

The same reasoning applies to variance swaps.
The fair strike 
$K_{\mathrm{var}}$
for the variance swap of 
maturity 
$T$
can, within our framework, be obtained 
by taking the expectation
$\EE_0[\Sigma_T]$.
It therefore follows from the concavity 
of the square root function and Jensen's 
inequality\footnote{For any convex function
$\phi:\RR\rightarrow\RR$
and any random variable 
$X:\Omega\rightarrow\RR$
with a finite first moment
Jensen's inequality states that
$\phi(\EE[X])\leq\EE[\phi(X)]$.}
that the following relationship holds  
between the fair strikes of the variance and 
volatility swaps
$$K_{\mathrm{vol}}<\sqrt{K_{\mathrm{var}}},$$
for any maturity
$T$.
This inequality is always satisfied by the market 
quoted prices for variance and volatility swaps and 
is there to account for the fact that variance 
is a convex function of volatility. Put differently, 
this is just a convexity effect, similar
to the one observed for ordinary call options, 
related to the magnitude of 
volatility of volatility. The larger the
``vol of vol'' is, the greater the convexity 
effect becomes. This phenomenon can be observed 
clearly in the markets with a very steep skew 
for implied volatilities. If one wanted to
estimate its size in general, it would be necessary to
make assumptions about both the level and 
volatility of the future realized volatility.
Within our model this can be achieved directly 
by comparing the values of the two expectations
(see figure~(\ref{fig:VarSwapTerm})
for this comparison based on the market implied 
vanilla surface for the S\&P 500).

There are other variance payoffs which are of practical
interest and can be
priced and hedged within our framework.
Examples are volatility and variance swaptions
whose payoffs are
$(\sqrt{\Sigma_T}-K_{\mathrm{vol}})^+$
and
$(\Sigma_T-K_{\mathrm{var}})^+$
respectively,
where as usual
$(x)^+$
equals
$\max(x,0)$
for any 
$x\in\RR$. 
Capped volatility swaps are also 
traded in the markets. Their payoff function is 
of the form
$(\min(\sqrt{\Sigma_T},\sigma_m) -K_{\mathrm{vol}})$,
where
$\sigma_m$
denotes the maximum allowed realized variance.
It is clear that all such contracts can be priced
easily within our framework by integrating any of these payoffs
against the probability distribution function (see
figure~\ref{fig:RealizedVar}
for maturities above 6 months)
of the annualized
realized variance
$\Sigma_T$
and then multiplying the expectation
with the corresponding discount factor.

It should be noted that there exist even more exotic
products, like corridor variance swaps (see~\cite{Carr2}), 
whose payoffs depend on the variance that accrues only
if the underlying is in a predefined range.
Such products cannot be priced  directly in 
the existing framework.
A modification of the model  
would be required to deal with this class of derivatives.
% The price of such a derivative could in principle be calculated 
% within the model by applying a partial Monte Carlo method to obtain
% the weights of the paths of the underlying that stay within the 
% range and then using the model to calculate the corresponding 
% pdfs for the realized variance.
However we will not pursue this avenue any further.


\subsection{Forward staring options and the volatility index}
\label{subsec:VIX}
Let 
$T'$
and
$T$
be a pair of maturities such that
$T'<T$.
A \textit{forward staring option} 
(or a \textit{forward-start}) is
a vanilla option with expiry
$T$
and the strike, set at time
$T'$,
which is equal to
$\alpha S_{T'}$.
The quantity 
$S_t$
is the underlying financial instrument 
the option is written on (usually a stock
or an index). More formally the value 
of a forward-start at time
$T$
(i.e. its payoff) is given by 
\begin{eqnarray}
\label{eq:FwdStartPayoff}
V_{FS}(T)=\left(S_T-\alpha S_{T'}\right)^+,
\end{eqnarray}
where the constant 
$\alpha$
is specified at the inception of the 
contract
and is know as the 
\textit{forward strike}. 
It is clear from the definition of the forward-start
that its value at time 
$T'$
equals the value of a plain vanilla call option
$$V_{FS}(T')=V_C(S_{T'},T-T',\alpha S_{T'})$$
that expires in 
$T-T'$
years and whose 
strike equals
$\alpha S_{T'}$.
Notice that at time
$T'$
the constant  
$\alpha$
can be characterized as the ratio\footnote{This
ratio is sometimes referred to as the ``moneyness''
of the option.}
between the spot price
$S_{T'}$
and the strike of the call option
into which the forward-start is transformed.
In the classical Black-Scholes framework, we have an 
explicit formula, denoted by
$\mathrm{BS}(S_{T'},T-T',\alpha S_{T'},r',\sigma')$, 
for the value of this call option (see~\cite{BS}).
This formula depends linearly on the spot level
$S_{T'}$
if the ratio of the spot and the 
strike (i.e. the ``moneyness'') is known.
In other words, assuming we are in the Black-Scholes 
world with a deterministic term-structure of volatility
and interest rates and zero dividends, 
we can express the value of the 
forward-start at time
$T'$
as 
$$V_{FS}(T')=S_{T'}\mathrm{BS}(1,T-T',\alpha,r',\sigma'),$$
where 
$\sigma'$
is the forward volatility rate\footnote{Assuming that
the term-structure of volatility is parametrized by
$\sigma(t)$,
the forward volatility rate 
$\sigma'$
is given by 
$\sigma'^2=\frac{1}{T-T'}\int_{T'}^T\sigma(t)^2dt.$}
and  
$r'$
is the forward interest rate between
$T'$
and
$T$.
The following key observations about the Black-Scholes value
and sensitivities of the forward-starting option are now clear:
\begin{itemize}
\item the value equals
      $V_{FS}(0)=S_{0}\mathrm{BS}(1,T-T',\alpha,r',\sigma')$
      and the delta 
      (i.e. $\frac{\partial}{\partial S_0}V_{FS}(0)$)
      is simply 
      $\mathrm{BS}(1,T-T',\alpha,r',\sigma')$,
\item the forward-starting option is gamma 
      neutral\footnote{It should be noted that, in the 
                       presence of stochastic volatility,
                       the gamma of a forward-starting option 
                       is no longer necessarily zero. However in 
                       a realistic model it should not be too 
                       large because it reflects
                       the dependence of volatility on very 
                       small moves of the underlying,
                       the effect of which should be negligible.}
      (i.e. $\frac{\partial^2}{\partial S_0^2}V_{FS}(0)=0$) 
      and 
\item the contract has non-zero vega (i.e.            
      $\frac{\partial}{\partial \sigma'}V_{FS}(0)>0$).  
\end{itemize}

We are interested in the Black-Scholes pricing formula
for the forward-starts because we need to use it when expressing
the forward volatility smile of our model. 
The values of forward volatility 
$\sigma'$,
implied by the equation
$V_{FS}(0)=S_{0}\mathrm{BS}(1,T-T',\alpha,r',\sigma')$,
are plotted in 
figures~\ref{fig:fs_skew3m},
\ref{fig:fs_skew6m}, \ref{fig:fs_skew1y} 
and~\ref{fig:fs_skew2y}
for a wide range of values of the forward strike
$\alpha$
and a variety of time horizons
$T',T$.
In other words, we first calculate the value 
$V_{FS}(0)$
of the forward-start and then 
invert the Black-Scholes pricing formula 
to obtain the implied forward volatility 
$\sigma'$.

We shall now give a brief description of 
the implied volatility index (VIX)
and then move on 
to discuss the future probability distribution of VIX,
which, as will be seen, is directly related to forward-starting 
options.

VIX was originally introduced in 1993 by Chicago Board Options Exchange 
(CBOE) as an index reflecting the 1 month implied volatility of the 
at-the-money
put and call options
on S\&P 100. 
To facilitate trading in VIX, 
in 2003 CBOE introduced a new calculation, using 
a full range of strikes for
out-of-the-money options, to define the value of VIX. At the same time
the underlying financial instrument on which the options are written 
was changed to S\&P 500
(for a detailed description of these changes and their ramifications
see~\cite{VIX}).
The new formula is 
\begin{eqnarray}
\label{eq:VixDef}
\sigma_{\mathrm{VIX}}^2=\frac{2}{T}\sum_i\frac{\Delta K_i}{K_i^2}e^{rT}Q(K_i)
-\frac{1}{T}\left(\frac{F}{K_0}-1\right)^2,
\end{eqnarray}
where the index itself is given by
$\mathrm{VIX}=100\sigma_{\mathrm{VIX}}$.
The sequence
$K_i$
consists of all the exchange quoted strikes and the quantities 
$Q(K_i)$
are the corresponding values of out-of-the-money 
put/call options expiring at maturity
$T$,
where 
$T$
equals 1 
month%\footnote{The actual CBOE definition of VIX uses two maturities,
% rather than one, 
% and the two corresponding strips of options.
% The value of  
% $\sigma_{\mathrm{VIX}}^2$
% is then defined to be 
% a convex combination of the two values given by 
% the formula in~(\ref{eq:VixDef}). Details of this construction 
% can be 
% found in~\cite{VIX}. We are going to
% neglect this technical point because its use is 
% mainly to circumvent
% certain market irregularities when dealing with 
% options with short time to expiry and does not add 
% complexity to
% the modelling side of the problem.}.
The quantity 
$F$
in formula~(\ref{eq:VixDef}) is the forward value 
of the S\&P 500 index derived 
from option prices\footnote{See page 3 in~\cite{VIX} for the precise definition.}
and the at-the-money strike
$K_0$
is defined as the largest strike below
$F$.
Note also that it is precisely at 
$K_0$
that 
the symbol
$Q(K)$
in~(\ref{eq:VixDef})
changes from put to call options. 

The reason why formula~(\ref{eq:VixDef})
allows easier trading of volatility follows 
from the simple observation that 
$\sigma_{\mathrm{VIX}}^2$
is
essentially the value of a European derivative,
expiring at time
$T$,
with the 
logarithmic payoff given in~(\ref{eq:LogDecom}).
This is a consequence of
the well-known decomposition of any twice
differentiable 
payoff described in~\cite{Breeden}, \cite{Carr}, \cite{Derman}
and other sources:
\begin{eqnarray}
\label{eq:LogDecom}
-\log\left(\frac{S_T}{F}\right)=-\frac{S_T-F}{F}+\int_0^F\frac{1}{K^2}(K-S_T)^+dK
+\int_F^\infty\frac{1}{K^2}(S_T-K)^+dK.
\end{eqnarray}
This formula holds for any value of 
$F$,
but expressions simplify if we assume that 
$F$
equals 
the forward of the index 
$S_t$
at time 
$T$
(i.e.
$F=\EE[S_T]$).
By taking the expectation with respect to the risk-neutral measure
we get the following expression for the forward price of the log payoff:
\begin{eqnarray}
\label{eq:VarHedge}
-\EE\left[\log\left(\frac{S_T}{F}\right)\right]
=\int_0^F\frac{1}{K^2}e^{rT}P(K)dK
+\int_F^\infty\frac{1}{K^2}e^{rT}C(K)dK,
\end{eqnarray}
where 
$C(K)=e^{-rT}\EE[(S_T-K)^+]$
(resp.
$P(K)=e^{-rT}\EE[(K-S_T)^+]$)
is the price of a call (resp. put) option struck at 
$K$.
It is shown  
in~\cite{Derman}
that the portfolio of vanilla options given by~(\ref{eq:VarHedge})
can be used to hedge perfectly a variance swap 
if there are no jumps in the underlying market.
From our point of view the expression~(\ref{eq:VarHedge})
is interesting because a simple calculation shows that 
definition~(\ref{eq:VixDef})
is a possible discretization of it. 
By defining its own version of the
approximation to the logarithm,
CBOE has created a volatility index which can be replicated by trading
a relatively simple European payoff. This feature greatly simplifies 
the  trading of VIX. 

Since the implied volatility index
is defined by a portfolio of puts and calls in~(\ref{eq:VixDef}), 
it is clear that the random nature of the value of
VIX 
at time
$t$
will be determined by
the value of the corresponding portfolio of
forward-starting options. 
The probability distribution
function for the behaviour of the volatility index at
$t$
is obtained from the model by the following procedure:
%\vspace{1mm}
\begin{enumerate}
\item[(I)]   Fix a level $S$ of the underlying.
\item[(II)]  Find the probability 
             that the price 
             process is at level
             $S$ at a given time 
             $t$
             in the future.
\item[(III)] Evaluate the portfolio of options 
             that define the volatility index 
             between times 
             $t$
             and
             $t+T$,
             conditional on the process 
             $S_t$
             being at level
             $S$.                
\item[(IV)]  Repeat these steps for all attainable
             levels
             $S$
             for the underlying Markov chain
             $S_t$.
\item[(V)]   Subdivide the real line into intervals with disjoint
             interiors of length
             $\delta$,
             where 
             $\delta$
             is a small positive number.
             To each of the intervals assign a probability 
             that is a sum of probabilities in step (II)
             corresponding to 
             the values obtained in step (III) that lie
             within the interval.          
\end{enumerate}
\vspace{1.5mm}
This describes the construction of the probability distribution
function of the volatility index at time 
$t$.
The plot of this pdf for a variety 
of maturities can be seen in figure~\ref{fig:VIXpdf}.

Our final task is to price any European payoff written on
the level of VIX at a certain time horizon. 
Given that our model allows us to extract
the pdf of VIX for any
expiry, pricing such a derivative amounts to integrating the 
payoff function against the probability distribution that was
described above.




==> model.tex <==
In this section we are going to describe the 
model for the underlying equity index
which we later calibrate to the implied 
volatility surface for vanilla
options on the S\&P 500 (see Section~\ref{sec:calibration}
and Figure~\ref{fig:ivols}).
Our model will be a mixture of local
and stochastic volatility coupled with an infinite
activity jump process
and will be defined on a 
continuous-time lattice in a largely non-parametric fashion.
The basic framework is 
an application to equity derivatives 
of the methods 
used in~\cite{FXrev} for modelling the foreign exchange rate. 
Our basic tools for all the 
constructions that follow will be spectral theory 
and numerical linear algebra.

We are assuming that, apart from the options data, we are also
given a term-structure of interest rates
and a continuously compounded deterministic
dividend schedule.
In other words interest rate
$r(t)$ 
and dividend yield 
$d(t)$ 
are given as deterministic functions of
calendar time 
$t$. 
Our modelling primitive will not be the equity
index
$S_t$
itself
but its forward price
$F_t =e^{(d(t)-r(t))t}S_t$.
Put differently, the model will be defined 
under the forward measure with the 
underlying process a martingale,
because,
on a lattice, 
it is numerically 
more convenient to simulate a stochastic 
process without drift (i.e. a martingale)
than one with a drift. 

The process
for the forward price $F_t$ will
be defined as follows. We shall first 
introduce a number of local volatility
regimes, all following CEV processes
with different parameter sets.
We will then add jumps to each of them 
using subordination
and then introduce the stochasticity
of volatility by specifying its dynamics so that
it is correlated to the level of the forward.  
In the rest of this section we will go through these
steps in more detail. In subsection~\ref{subsec:CondPDF}
we will address the issue of the pricing and hedging of
European derivatives and forward-starting options.

\subsection{The local volatility processes.}
\label{subsec:LocalVol}
Our model will comprise $M$ local volatility regimes
(in order to fit the implied volatility 
surface for the S\&P 500, we used 
$M=2$
regimes). 
The switching between the volatility regimes 
will be driven by a stochastic process, which will be correlated
with the level of the forward price $F_t$. This construction
will be carried out in subsection~\ref{subsec:StochVol}.

As mentioned 
above, all these local volatility regimes will be from the same
class, namely that of CEV processes. We are now going to define 
a continuous-time Markov chain, which is a discretization
of a generic CEV process. The family of local volatility
processes will then be obtained by judiciously choosing
a family of the CEV parameters. 

Recall that 
forward price 
$F_t$ 
can be defined 
as a CEV process by the following stochastic differential
equation
\begin{equation}
\label{eq:lv}
d F_t = v(F_t) dW_t, \>\>\>\mathrm{where}\>\>\> 
v(F_t):= F_{t} \min( \sigma F_{t}^{\beta-1},\bar\sigma) 
\end{equation}
and where
$W_t$
is the standard Brownian motion. The capping constant
$\bar\sigma$
was introduced into this definition of the CEV process 
in order to avoid accumulation of probability 
at the boundary of the domain of the 
process
$F_t$.
It is well-known
(e.g. see chapter 5 in~\cite{Karatzas})
that the Markov generator 
of a diffusion process 
given by the stochastic differential equation~(\ref{eq:lv}) 
acts in the following way on any twice differentiable
real function 
$\phi$:
\begin{eqnarray}
\label{eq:MG}
(\L\phi)(F) = \frac{v(F)^2}{2} 
\frac{\partial^2\phi}{\partial F}(F).
\end{eqnarray}
The probability density function
$p(G,t;F,T)=\PP(F_T=F\vert F_t=G)$
is the solution of the partial differential equation
$$\frac{\partial p}{\partial t}+\L p=0$$
with boundary condition 
$p(G,T;F,T)=\delta(G-F)$,
where 
$\delta$
is the Dirac delta function.
This PDE is known as the \textit{backward Kolmogorov equation}
for the process 
$F_t$
and it implies that all the information required to
obtain the 
probability kernel
$p(G,t;F,T)$
is contained in the Markov generator given by~(\ref{eq:MG}). 
For this reason
we will define the probability kernel of the continuous-time
Markov chain that will approximate the 
process 
$F_t$
using a natural discretization of the Markov 
generator
$\L$.

In order to define this dynamics we must first 
define a discrete domain 
for the forward rate
$F_t$
which can be achieved as follows.
Let 
$\Omega$
be a finite set 
$\{0,\ldots,N\}$
containing 
the first 
$N$ 
integers together with
$0$
and let 
$ F:\Omega\rightarrow \RR $
be a non-negative function which satisfies the following
two conditions:
$F(0)\geq0$
and
$F(x)>F(x-1)$
for all 
$x$
in
$\Omega-\{0\}$.
Given such a function 
$F$,
the discretized forward rate process 
$F_t^\Omega$
can take any of the values 
$F(x)$,
where 
$x$
is an element in
$\Omega$
and time
$t$
is smaller than some time horizon
$T$.

The next step is to ensure that the dynamics of 
the discretized 
forward process correspond to the dynamics specified
by the stochastic differential
equation~(\ref{eq:lv}). As mentioned above this will now be  
achieved by reinterpreting the Markov generator~(\ref{eq:MG})
in the discrete setting. 
Note first that the differential operator
$\L$
is just the Laplace operator
multiplied by a scalar function.
A natural discretization of
the Laplace operator is given by 
\begin{eqnarray}
\label{eq:DiscreteLaplace}
(\Delta^\Omega u)(x):=
\left\{\begin{array}{ll}
       u(x+1)+u(x-1)-2u(x) & \mbox{if $x \in\Omega-\{0,N\}$,} \\
                         0 & \mbox{otherwise,} 
                      \end{array}
               \right.
\end{eqnarray}
for all functions 
$u$
on 
$\Omega$.
Note that this definition of the discretized Laplace operator 
imposes absorbing boundary conditions
on the Markov chain, associated to
$\Delta^\Omega$,
at each end of the domain
$\Omega$.
This is a reasonable requirement of the underlying process
for two reasons. Firstly, since the size of the set 
$\Omega$
is a parameter of our model, we can make sure that 
it is of sufficient size 
so that we can calibrate to the market data
without the process ever reaching the boundary. Secondly,
this choice of boundary conditions makes it easy to detect
if the domain 
$\Omega$
is not large enough, which would not necessarily be the case 
had we used reflecting boundary conditions\footnote{The 
choice of the boundary behaviour of a Markov chain representing 
the realized variance of the underlying 
will be of fundamental importance in Sections~\ref{sec:path} and~\ref{sec:Bloc}.
There however, a different, perhaps slightly
unnatural, boundary condition will be most useful.}.

Let the operator
$\L^\Omega$
denote the discretized version of the generator
$\L=\frac{v^2}{2} \Delta$.
Using the discrete version of the Laplace 
operator~(\ref{eq:DiscreteLaplace}),
we can define the generator
$\L^\Omega$
as a tridiagonal matrix
of size
$(N+1)\times(N+1)$ 
with entries
$\L^\Omega(x,y)$,
where
$x$
and 
$y$
are elements of 
$\Omega$,
that satisfy the following conditions for all 
$x$
in
$\Omega$:
\begin{eqnarray}
  \label{eq:ProbConserv}
  \sum_{y\in\Omega} \L^\Omega(x,y) &=& 0, \\
  \label{eq:martingale}
  \sum_{y\in\Omega} \L^\Omega(x,y) (F(y)-F(x)) &=& 0, \\
  \label{eq:InstantaneousVariance}
  \sum_{y\in\Omega} \L^\Omega(x,y) (F(y)-F(x))^2 &=& v(F(x))^2.
\end{eqnarray}
 
Condition~(\ref{eq:ProbConserv}) is there to secure 
probability conservation over the
infinitesimal time interval $dt$
and stems from the fact that a generator
of a continuous-time Markov chain consists
of the gradients of probability for jumping 
from any point 
$x\in\Omega$
to any other point 
$y\in\Omega$. 
Therefore equation~(\ref{eq:ProbConserv}) is simply a derivative of the
equation
$\sum_{y\in\Omega}\PP(F_s^\Omega=F(y)\vert F_t^\Omega=F(x))=1$
with respect to 
$s$
at time
$t$.
The second  and the third conditions
are the instantaneous\footnote{It is well-known that
the first two instantaneous moments
of any diffusion determine its finite-dimensional
distribution functions completely (see~\cite{Karatzas}). 
It is therefore sufficient
for the process
$F_t^\Omega$
to match these two conditions 
in order to be a valid approximation
of
$F_t$.}
first and second moment-matching 
conditions for the discretized process
$F_t^\Omega$.
Equality~(\ref{eq:martingale})
is a martingale condition for
$F_t^\Omega$
since the process
$F_t$
has no instantaneous drift.
Condition~(\ref{eq:InstantaneousVariance})
guarantees that the Markov chain has the same instantaneous
variance as the diffusion defined by the SDE in ~(\ref{eq:lv}).

The final constraint in the construction of the Markov generator
$\L^\Omega$
comes from the specification of the process at the boundary
of its domain.
We would like to ensure that the process
$F_t^\Omega$
obeys absorbing boundary conditions whenever it gets that far.
As discussed above, this can be done by setting 
all elements in the top and bottom row of the matrix
$\L^{\Omega}$
to be equal to zero. In coordinates this can be expressed by
the condition 
$$\L^{\Omega}(x,y)=0,\>\>\>\mathrm{for}\>\>\mathrm{all}\>\>\>
y\in\Omega,\>\>x\in\{0,N\}.$$
Notice that this operation does not interfere with 
conditions~(\ref{eq:ProbConserv}), (\ref{eq:martingale})
and~(\ref{eq:InstantaneousVariance})
and hence gives us a well-defined generator for the Markov
process 
$F_t^\Omega$.

\subsubsection{Computing the probability kernel}
\label{sub:ProbKernel}
Our next task is to obtain the probability kernel of the 
process 
$F_t^\Omega$
from its Markov generator
$\L^\Omega$. 
This can be achieved for very general Markov processes by applying spectral
methods of operator theory. 
Here we will only illustrate 
the spectral resolution method in the
special case of the finite-dimensional matrix 
$\L^\Omega$.
This method is sufficient for our purposes
and 
can be applied directly to other cases which are of interest
to us, such as 
the introduction of jumps (see
subsection~\ref{subsec:Jumps}) and the calculation
of the probability kernel for the realized variance
of the underlying process (see Section~\ref{sec:pricing}). 
We start by considering the following eigenvalue
problem
\begin{eqnarray}
\label{eq:DiagProb}
\L^\Omega u_n = \lambda_n u_n
\end{eqnarray}
for the matrix
$(\L^\Omega(x,y))_{x,y\in\Omega}$.
The vectors
$u_n$ 
are the eigenvectors 
of the linear operator 
$\L^\Omega$
and the scalars $\lambda_n$ are the
corresponding eigenvalues. 
Except in trivial cases, the Markov
generator 
$\L^\Omega$ 
will not be a symmetric matrix, which implies that 
the zeros of the characteristic polynomial of
$\L^\Omega$
(i.e. the eigenvalues
$\lambda_n$)
will not be real. On the other hand
it is not hard to see that an element
$\lambda_n$
of the spectrum of
any Markov generator
must have a 
non-positive real part 
(${\mathcal Re}(\lambda_n) \leq 0$)
and that the
complex eigenvalues occur in conjugate pairs (i.e.
$\lambda_n$ is an eigenvalue if and only if $\overline{\lambda_n}$ is
an eigenvalue).

In general of course, there is no guarantee that there exists a
complete set of 
$(N+1)$
eigenvectors
$u_n$
for the operator
$\L^\Omega$.
However, such a set will certainly exist if
we can find 
$(N+1)$
distinct eigenvalues
$\lambda_n$
of
$\L^\Omega$.
But the set of all 
$(N+1)\times(N+1)$
matrices 
which do not have distinct eigenvalues 
must have Lebesgue measure zero
for the same reason that the set of all polynomials of order
$(N+1)$
with at least two coinciding zeros has Lebesgue measure zero.
Therefore
the chance that such a
complete set does not exist, for a Markov generator specified
in a
nonparametric fashion 
is zero, so we can safely assume that the complete set
of eigenvectors exists.
In the unlikely event that this assumption is not valid, the
numerical linear algebra routines needed to solve our lattice model
will identify the problem and an arbitrarily small perturbation of 
a given operator will suffice to rectify the situation. Assuming
that there is a solution, the diagonalization 
problem~(\ref{eq:DiagProb}) can be 
rewritten in the
following matrix form
$$\L^\Omega = U\Lambda U^{-1},$$
where 
$U$ 
is the matrix whose columns are the eigenvectors 
$u_n$
and
$\Lambda$ is the diagonal matrix with the eigenvalues 
$\lambda_n$.

Key to our constructions is the remark that, if the Markov generator
is diagonalizable, we can apply to it an arbitrary function 
$\phi$,
defined on the spectrum of the generator,
by means of the following formula:
\begin{equation}
\label{eq:FF}
\phi(\L^\Omega) = U \phi(\Lambda) U^{-1}.
\end{equation}
The expression~(\ref{eq:FF}) is useful because
the task of calculating  
$\phi(\Lambda)$
is a very simple one:
\[\phi(\Lambda) = 
\begin{pmatrix}
            \phi(\lambda_0) & \cdots & 0 \\
            \vdots & \ddots &  \vdots \\
            0 & \cdots & \phi(\lambda_N)
\end{pmatrix}.
\]      

It can be seen by a direct calculation (see chapter 6 
in~\cite{Grimmett}) that the matrix
$P_t=e^{(T-t) \L^\Omega}$
satisfies the backward Kolmogorov equation,
much like the one for the original diffusion,
\begin{eqnarray}
\label{eq:DiscKolmog}
\frac{\partial P_t}{\partial t}+\L^\Omega P_t=0
\end{eqnarray}
with the boundary condition
$P_T=\II$,
where
$\II$
denotes the identity matrix on the vector space
$\RR^{N}$.
This fact, combined with formula~(\ref{eq:FF}),
gives us an explicit expression for the transition
probability kernel of 
$F_t^\Omega$:
$$\PP(F_T^\Omega = F(y) \lvert F_t^\Omega = F(x)) = 
(e^{(T-t) \L^\Omega})(x,y) =
\sum_{n=0}^N e^{\lambda_n (T-t)} u_n(x) v_n(y).$$
In this expression the vectors
$v_n$
correspond to the columns of the matrix
$U^{-1}$.

%-------------------------------------------------------------------------

\subsection{Adding jumps}
\label{subsec:Jumps}

As defined so far the Markov chain
$F_t^\Omega$
behaves like a 
pure diffusion process. It is known that this class
of models is not well suited to explain the volatility skew
for options with short maturity because of the extremely small 
probabilities of large moves in the underlying in short-time horizons.
In the equity markets however, jumps are commonplace
and as such they influence the prices of short-dated out-of-the-money options.
If we want to calibrate our model to the entire volatility surface
we therefore need to introduce jumps into the risk-neutral dynamics 
of the underlying forward rate
$F_t^\Omega$.
Using spectral theory this can be easily achieved in a general way.
What we want is to have different distributions of jump sizes for jumps
up and jumps down. Having this property in our model is crucial because
the market expectations for jumps up and down are know to the market
makers and are almost always very different from each other. Therefore,
any process that aspires to model the risk-neutral dynamics of the 
underlying correctly
must be able to account for this difference. 
The variance-gamma model, defined in~\cite{MCC}, has this property 
since the characteristic function 
of the underlying process\footnote{The process used in~\cite{MCC} 
is a time-changed Brownian motion with drift. The stochastic
time is given by a gamma process.}
is not real.

A general way of building infinite-activity  
jump processes is by subordinating
diffusions using a special class of stochastic time
changes. 
Such a time change is given by a non-decreasing 
stationary process
$T_t$ 
with independent increments. The time change
$T_t$
is known as a
\textit{Bochner subordinator} 
and is characterized by a \textit{Bernstein function}
$\phi(\lambda)$ 
which has the following property
$$ E_0\left[e^{-\lambda T_t} \right] = e^{-\phi(\lambda)t}.$$
In other words the process
$T_t$
is a non-decreasing stationary process 
with independent increments whose Laplace transform 
takes the special form
$e^{-\phi(\lambda)t}$,
where 
$\phi(\lambda)$
is the Bernstein function of the process.
 
For example in the case of the afore mentioned variance-gamma process, 
the Bernstein function is of the form 
\begin{eqnarray}
\label{bochner}
\phi(\lambda) =
\frac{\mu^2}{\nu}\log\left(1+\lambda\frac{\nu}{\mu}\right).
\end{eqnarray}
The parameter 
$\mu$ 
is the mean-reversion rate
(usually taken to be equal to
1) and 
$\nu$ 
is the variance rate of the
variance-gamma process. 

It was shown in~\cite{Phillips}
that, given a general Markov process
$X_t$
with a generator
$\L$
and a Bochner subordinator
$T_t$,
the subordinated process
$X_{T_t}$
is a Markov process with a generator
$\L'=-\phi(-\L)$,
where 
$\phi$
is the Bernstein function of
$T_t$.

In our framework we need to add jumps to the 
local volatility process 
$F_t^\Omega$
given by the generator
$\L^\Omega$.
In order to produce asymmetric
jumps we specify two Bernstein functions 
of the variance-gamma process by choosing two
jump intensities
$\nu_+$
for up and
$\nu_-$
for down.

We then compute separately the two Markov
generators
$$ \L_\pm = -\phi_{\pm}(-\L^\Omega) = -
U_{\pm}\phi_\pm(-\Lambda) U^{-1}_{\pm},$$
where 
$\Lambda$
is the diagonal matrix from subsection~\ref{sub:ProbKernel}
and the Bernstein functions 
$\phi_\pm$
are given by
$$\phi_{\pm}(\lambda) =
\frac{1}{\nu_{\pm}}\log(1+\lambda\nu_{\pm}).$$

Each of the square matrices
$\L_\pm$
corresponds to a time-changed diffusion process. In particular
the elements of
$\L_+$,
which are above the diagonal, 
are the (scaled) probabilities of jumping up in the infinitesimal
time interval 
$dt$.
On the other hand, the sub-diagonal triangle of 
$\L_-$
contains the (scaled) probabilities of jumping down in the time interval
$dt$.
Thus we can define a new generator for our process, which will have 
asymmetric jumps,
by combining the two generators in the following way
\[
\L^\Omega = \begin{pmatrix}
d(0,0) & \L_+(0,1) & \cdots & \L_+(0,N-1) & \L_+(0,N)  \\
\L_-(1,0) & d(1,1) & \cdots & \L_+(1,N-1) & \L_+(1,N) \\
\vdots & \vdots  & \ddots & \vdots & \vdots\\
\L_-(N-1,0) & \L_-(N-1,1) & \cdots & d(N-1,N-1) & \L_+(N-1,N) \\
\L_-(N,0) & \L_-(N,1) & \cdots & \L_-(N,N-1) & d(N,N) 
\end{pmatrix}.
\] 

Since we want our new process with jumps to be a martingale, we need to
make sure that condition~(\ref{eq:martingale}) is satisfied for the
new generator
$\L^\Omega$.
This can be done easily by adjusting 
the elements just above and below the diagonal of the matrix
$\L^\Omega$.
If for example the drift in the  
$x$-th 
row of 
$\L^\Omega$
is positive, we add some probability to the element 
$\L^\Omega(x,x-1)$
so that the condition~(\ref{eq:martingale}) becomes valid.
If, on the other hand, 
the drift in the  
$x$-th 
row is negative, then we can help the generator pull up the process
by adding probability to the element
$\L^\Omega(x,x+1)$.
Once we do this for all 
$x$,
the new modified operator, which we again call
$\L^\Omega$,
will satisfy the martingale condition in~(\ref{eq:martingale}). 

A possible undesirable effect of subordination 
on the underlying process
is a linear deterministic time change (along with the 
stochastic one). This would result in the distortion of the instantaneous
variance of the underlying process by a constant factor. In order 
to avoid this effect, we multiply each row of the subordinated generator
by a constant chosen in such a way, so that 
equation~(\ref{eq:InstantaneousVariance}) holds.
Since the function
$v(F(x))$
on the righthand side of~(\ref{eq:InstantaneousVariance})
gives the value of the instantaneous variance of the local
volatility process we started with, this procedure eliminates
the linear deterministic time change that might have occurred
during subordination. Notice also that the rescaling of the rows
of 
$\L^\Omega$
has preserved the martingale condition in~(\ref{eq:martingale}),
which has been manufactured above.   

The procedures we have just carried out did not require the 
knowledge of the diagonal elements of
$\L^\Omega$.
They need to be chosen in such a way that
the probability conservation (condition~(\ref{eq:ProbConserv})) 
is satisfied.
This can be achieved by simply defining 
the diagonal elements in the following way
$$ d(x,x) = - \sum_{y \in \Omega-\{x\}} \L^\Omega(x,y).$$
This gives us a well-defined Markov generator
$\L^\Omega$
for a diffusion process with jumps, 
which can be used to model 
the risk-neutral forward rate because it is a martingale, and 
whose instantaneous variance has not been altered by 
subordination.

The construction we have just presented 
differs in two ways from the one in~\cite{MCC}. Firstly 
our time-changing approach is applicable to
a general diffusion process which need not be 
translation invariant\footnote{A key feature of L\'{e}vy 
processes is that they are translation invariant. That is precisely the
property of the Brownian motion with a drift required in the 
construction of the jump process in~\cite{MCC}.}. 
Secondly we have the additional 
flexibility of specifying explicitly the intensities of up-jumps and 
down-jumps separately. 

%-----------------------------------------------------------------------------

\subsection{Modelling the dynamics of stochastic volatility}
\label{subsec:StochVol}

In order to introduce the stochasticity of volatility 
into our modelling framework, we need to start with
$M\in\NN$
jump-diffusions of subsection~\ref{subsec:Jumps}
(all defined on the same
domain
$\Omega$)
which are given by Markov generators
$\L_\alpha^\Omega$
for
$\alpha=0,\ldots,M-1$.
In this subsection we are going to define
the dynamics of stochastic volatility
that will give our model the ability to switch between the
various jump-diffusion regimes. As will
become clear, the stochasticity of volatility
will be sensitive to the current level of the underlying,
thus making it possible to relate the model to
a particular view of the market. It is not uncommon among 
market participants to express market views (i.e. skew and 
smile behaviour of option prices) in terms of
the future 
``levels'' at which the underlying might be trading.
In our framework we can set these levels
explicitly and are allowed to choose independently
the corresponding jump-diffusion, that can express 
the required view of the volatility surface.
The introduction of stochastic volatility into the model 
will be in several stages. 
Let us start by specifying the dynamics of stochastic volatility
and then combining them with the underlying jump-diffusion
regimes
to give a full specification of the model. 

Let
$V$
be the set
$\{0,\ldots,M-1\}$
of all possible volatility states.
For each volatility state
$\gamma$
(in
$V$)
we define a Markov generator
$\G^V_\gamma$
by specifying the matrix elements
$\G^V_\gamma(\alpha,\beta)$,
for all
$\alpha,\beta\in V$,
so that the continuous-time
diffusion given by
$\G^V_\gamma$
mean-reverts to one of the volatility states
in
$V$.

We have defined 
$M$
Markov generators
$\G^V_\gamma$, 
each of them specifying
its own dynamics of the stochastic volatility process.
Our next task is to obtain a single global stochastic
volatility Markov generator which will favour a certain
regime
$\gamma$
conditional on the position of the forward rate.
This can be achieved by using a \textit{partition of unity}
which is described as follows. Choose a strictly increasing 
sequence
$F_\gamma$
of the forward rate levels so that, if the forward process
is close to the
level
$F_\gamma$,
the market views of the smile and skew agree with the ones implied
by the process 
$\L^\Omega_\gamma$ from subsection~\ref{subsec:Jumps}. The partition
of unity is defined as a sequence of 
$M$
functions
$\epsilon_\gamma:\RR\rightarrow[0,1]$
with the key property
$$\sum_{\gamma=0}^{M-1}\epsilon_\gamma(F)=1, \>\>\>\mathrm{for}\>
    \mathrm{all}\>\>\>
F\in\RR.$$
Given the sequence of levels
$F_\gamma$, 
such functions can be defined explicitly, using
a piecewise linear scheme, in
the following way:
$$ \epsilon_\gamma(F) := \left\{\begin{array}{ll}
   \frac{F-F_{\gamma-1}}{F_{\gamma}-F_{\gamma-1}} & 
                  F\in[F_{\gamma-1},F_{\gamma}] \\
   \frac{F_{\gamma+1}-F}{F_{\gamma+1}-F_{\gamma}} & 
                  F\in[F_{\gamma},F_{\gamma+1}] \\
                         0 &  \mathrm{otherwise}.
%                          F\leq F_{\gamma-1}\>\> \mathrm{or} \>\>
%                               F\geq F_{\gamma+1}.
                          \end{array}
                        \right. $$
This definition has to be modified slightly for the boundary cases
when 
$\gamma$
equals 
$0$
or
$(M-1)$:
$$ \epsilon_0(F) := \left\{\begin{array}{ll}
                       1 & F\leq F_0 \\
   \frac{F_1-F}{F_1-F_0} & F\in[F_0,F_1] \\
                       0 & F\geq F_1,
                          \end{array}
                        \right. \>\>\>\>\>\>
\epsilon_{M-1}(F) := \left\{\begin{array}{ll}
                       0 & F\leq F_{M-2} \\
   \frac{F-F_{M-2}}{F_{M-1}-F_{M-2}} & F\in[F_{M-2},F_{M-1}] \\
                       1 & F\geq F_{M-1}.
                          \end{array}
                        \right. $$
We are now in a position to define our global Markov generator
for the stochastic volatility process, which has the capability of
changing its properties when the forward rate undergoes a substantial 
move. The definition, using the partition of unity,
goes as follows
$$\L^V_x(\alpha,\beta):=
\sum_{\gamma=0}^{M-1}\epsilon_\gamma(F(x))\G^V_\gamma(\alpha,\beta),$$
where
$\alpha, \beta$
are elements in
$V$
and 
$F(x)$
is the function on
$\Omega$
describing the forward rate process. It follows from the 
defining property of partition of unity that the matrix
$\L^V_x$
is indeed a Markov generator for any element
$x$
of the underlying space 
$\Omega$.

Just like with any stochastic volatility model,
our aim is to define a Markov generator
$\L$
which will specify the probabilities of going from
any state
$(x,\alpha)$
in
$\Omega\times V$
to any other state 
$(y,\beta)$
(of the same set)
in the infinitesimal time interval
$dt$.
% In order to do this we need the
% \textit{Kronecker delta} function which can be defined 
% on a cartesian product of any discrete set with itself,
% in the following way
% $$ \delta_{xy}=\left\{\begin{array}{ll}
%                          1 & \mbox{if $x = y$,} \\
%                          0 & \mbox{otherwise.}
%                       \end{array}
%                \right. $$
The Markov generator 
$\L$
that specifies the dynamics of our model for the underlying forward rate
is given by
\begin{eqnarray}
\label{eq:UnderlyingGen}
\L(x, \alpha; y, \beta) := \L^\Omega_{\alpha}(x,y) 
\delta_{\alpha\beta} + \L^V_x(\alpha, \beta)
\delta_{xy},
\end{eqnarray}
where 
$\delta$
denotes the Kronecker delta function.
Note that it follows trivially,
from the properties of the Kronecker delta, that the
matrix
$\L$
is a genuine Markov generator (i.e. it has positive entries off the diagonal
and its rows sum to one). 
Another important feature is that the generator
$\L$,
by definition, does not allow for simultaneous jumps of the 
state and the volatility variables. This property 
ensures that our
forward process 
$F_t^\Omega$,
whose dynamics is specified by 
$\L$,
remains a martingale:
\begin{eqnarray*}
\EE_t^{(x, \alpha)}[dF^\Omega_t] & = & \sum_{(y,\beta)\in\Omega\times V}
                                       \left(F(y)-F(x)\right)
                                       \left(
                                       \L^\Omega_{\alpha}(x,y)
                                       \delta_{\alpha\beta} + 
                                       \L^V_x(\alpha, \beta)
                                       \delta_{xy}\right) \\
                   & = & \sum_{y\in\Omega}     
                         \left(F(y)-F(x)\right)
                         \L^\Omega_{\alpha}(x,y) + 
                         \left(F(x)-F(x)\right)\sum_{\beta\in V}      
                         \L^V_x(\alpha, \beta) = 0. 
\end{eqnarray*}


%----------------------------------------------------------------------

\subsection{Deterministic time-change}
\label{subsec:DetTimeC}

The model we have described so far is completely stationary. 
This amounts to the fact that the implied volatility surface 
is influenced purely by the model parameters and 
has no explicit time dependence. By adjusting these parameters
one can obtain a general shape of the market impled volatility surface
and reprice correctly the out-of-the-money skew
(i.e. the difference between an out-of-the-money 
call and an out-of-the-money put). 

In order to get a good match for the term structure
of the at-the-money implied volatilities 
we have to introduce a minimal deterministic
time-change,
which only has a marginal effect on the out-of-the-money options.
This adjustment can be specified by an increasing function
$f:[0,T]\rightarrow[0,\infty)$ 
which deterministically
transforms calendar time 
$t$ 
to financial time 
$f(t)$. 
Since our
model can capture well the features of the underlying market before
the deterministic time-change is introduced, the calendar time 
$t$
and the financial time 
$f(t)$ 
will differ only slightly from each other.
We first find values of the function 
$f$
for all market specified maturities by satisfying the
requirement that the at-the-money options are
priced correctly. It will become clear in 
subsection~\ref{subsec:CondPDF}
that a deterministic time-change plays a very isolated role
in the pricing algorithm. Therefore finding a correct value
of
$f$
at the market specified maturities is not a difficult task.
For all other times 
$t$
we use a linear interpolation to arrive at the value
$f(t)$.  
The graph of the function
$f$,
used to calibrate the model to the market implied 
volatility surface for S\&P 500, is given in
Figure~\ref{fig:timechange}.

%----------------------------------------------------------------------

\subsection{Pricing and hedging of vanilla options and forward-starts}
\label{subsec:CondPDF}

The pricing problem for a general European 
option expiring at time
$T$ 
reduces to the calculation
of the transitional probability density function
$p((x,\alpha),t;(y,\beta),T)$
for the underlying process
$F_t^\Omega$,
which was defined in
subsection~\ref{subsec:StochVol}
via its Markov generator~(\ref{eq:UnderlyingGen})
(recall that 
$(x,\alpha),(y,\beta)$
are elements of
$\Omega\times V$
while
$t$
is the current time).
This is because our framework is defined in the risk-neutral
measure which implies that the value of any security
at time 
$t$
equals the discounted expectation of the value 
of the same security at any time horizon
$T$.

Since we would like to include the deterministic time-change
of subsection~\ref{subsec:DetTimeC}
in the definition of the density
$p((x,\alpha),t;(y,\beta),T)$,
we must start by specifying the 
risk-neutral dynamics of the underlying forward
process in financial time.
More precisely let
$$U_s=
(u((x,\alpha),s;(y,\beta),S))_{(x,\alpha),(y,\beta)\in\Omega\times V}$$
be a stochastic matrix induced by the Markov generator
$\L$.
In other words the coordinate functions 
$u((x,\alpha),s;(y,\beta),S)$
are the transition probabilities to go between the states
$(x,\alpha)$
and
$(y,\beta)$ 
in the time interval
$[s,S]$.
The quantity 
$s$
denotes the financial time
and can therefore be expressed as
$s=f(t)$,
where
$f$
is the function from subsection~\ref{subsec:DetTimeC}
and 
$t$
is the calendar time.
Similarly
$S=f(T)$
is the financial time horizon.

As was mentioned in subsection~\ref{subsec:LocalVol},
the matrix 
$U_s$
satisfies the backward Kolmogorov\footnote{Notice
that the Markov generator
$\L$
in this equation
acts on the coordinate functions of
$U_s$
as a function of the variable  
$(x,\alpha)$.}
equation~(\ref{eq:DiscKolmog})
with the boundary condition
$U_S=\II$
($\II$
is the identity matrix on the vector space
$\RR^{k}$
where
$k=M(N+1)$).
The solution of the backward Kolmogorov
equation can therefore be expressed in 
terms of functional calculus as
$U_s = \exp((S-s)\L)$
and can be calculated explicitly
using the spectral decomposition
of the operator
$\L$
(which in this case is just
$k\times k$ 
matrix)
as given by~(\ref{eq:FF}).
The first step is to calculate the eigenvalues
$\lambda_n$ 
of the Markov generator
$\L$
and the second is to find the eigenvectors 
$u_n$
of 
$\L$,
put them into a transition matrix
$U$,
and find the columns of the inverse
$U^{-1}$
which we will denote by
$v_n$.
In Section~\ref{sec:calibration}
we calibrate the model using a lattice
with
$M(N+1) = 2\cdot 76 = 152$
points
which implies that the generator
$\L$ 
is a square matrix of dimension
$152\times152$.
For matrices of this size diagonalization
routines such as {\tt dgeev} in the numerical
linear algebra library LAPACK are very efficient.

Once we have the spectral decomposition of
$\L$,
we can calculate the probability kernel
$p((x,\alpha),t;(y,\beta),T)$, 
which depends on 
calendar time, using functional calculus:
\begin{equation*}
%\label{eq:kernel}
p((x,\alpha),t;(y,\beta),T)= 
e^{(f(T)-f(t))\L}((x,\alpha),(y,\beta)) =
\sum_{n=1}^{M(N+1)} e^{\lambda_n (f(T)-f(t))} u_n(x,\alpha) v_n(y,\beta).
\end{equation*}
Since we know that eigenvalues
$\lambda_n$
must have a negative real part, in the case of long-dated options
only very few eigenvalues will play a role, because the exponential
of a negative number becomes negligibly small very quickly.
Another surprising and important fact which follows 
from the above representation of the probability
kernel is that it
depends in a very isolated way on the (financial) time to maturity.

The current price
$C_t$
of a European derivative paying
$h(S_T)$
at the time horizon
$T$,
where 
$S_t$
is the underlying equity index,
can be calculated in the following way
\begin{eqnarray}
\label{eq:EuroPrice}
C_t(x,\alpha)=e^{-(r(T)T-r(t)t)}\sum_{(y,\beta)\in\Omega\times V}
p((x,\alpha),t;(y,\beta),T)h(e^{-(r(T)-d(T))T}F(y)).
\end{eqnarray}
The point 
$x$
from
$\Omega$
is chosen in such a way so that the equation
$F(x)= e^{(r(t)-d(t))t}S_t$
holds,
where 
$S_t$
is the index level at the current time  
$t$,
and 
$\alpha$
in
$V$
corresponds to the volatility regime we are in at time
$t$.

Our next task is to 
find the hedge-ratios for the derivative 
$C_0$
within our model.
It emerges that  this 
is a very simple matter which is not at all computationally demanding 
because all the hard numerical work has already been done 
by the pricing algorithm. 
The delta and the 
gamma of 
$C_0$
are defined using symmetric differences
in the following way
\begin{eqnarray*}
\Delta(x,\alpha) & := & 
               \frac{C_0(x+1,\alpha)-C_0(x-1,\alpha)}{F(x+1)-F(x-1)} \\
\Gamma(x,\alpha) & := &  
   4 \frac{C_0(x+1,\alpha)+C_0(x-1,\alpha)-2C_0(x,\alpha)}{(F(x+1)-F(x-1))^2},
\end{eqnarray*}
where 
$x$
is the lattice point in
$\Omega$
that corresponds to the spot level of the index
at time 
$0$
(note that at time 
0
the spot is the same as the forward).
Notice that calculating 
$C_t(x+1,\alpha)$,
or any other value of the option 
$C_t(y,\alpha)$
with a starting point 
$y$
different
from
$x$,
requires no further diagonalization because the pdf
we need is given by a different row of the matrix
$U_s$,
which has already been calculated during the pricing of the original
contract
$C_t(x,\alpha)$.
In fact if one requires the entire 
delta and gamma profiles of the derivative
$C_t$
(like the ones plotted in Figures~\ref{fig:DeltaCall}
and~\ref{fig:GammaCall}
for call options struck at 100),
the most efficient way of doing it is to use a general
matrix-vector multiplication routine 
{\tt gbmv} from LAPACK
and then piece together the corresponding Greeks 
using the above formulae.

A similar procedure can be applied to obtain the vega of the contract
$C_t$.
Again we can define it using a symmetric difference (in the stochastic
volatility domain
$V$)
with a formula
$$\nu(x,\alpha):= \frac{C_0(x,\alpha+1)-C_0(x,\alpha)}{\sigma_{\alpha+1}-\sigma_{\alpha}},$$
that needs to be suitably amended in case we are 
in the volatility regime on the boundary of the domain
$V$.
The parameters
$\sigma_\alpha$,
for 
$\alpha$
in the domain
$V$,
are the base volatilities in the CEV processes defined in
subsection~\ref{subsec:LocalVol}. Their values can be found
in table~\ref{t:para}.
It is clear that the same computational technique which yielded 
delta and gamma profiles can be used to find the vega profile
of the derivative
$C_t$
(see Figure~\ref{fig:VegaCall} 
for the vega profile of call options with different maturities
struck at 100).

Our final task is to find an algorithm for pricing
forward-starting options. Recall from subsection~\ref{subsec:VIX} 
that the payoff of a forward-start is of the form
$\left(S_T-a S_{T'}\right)^+$,
where 
$T'<T$
are a pair of maturities and 
$a$
is the forward strike.
Let us now assume that the current time is 
$0$
and let us reinterpret the formula~(\ref{eq:EuroPrice}),
for 
$t=T'$,
as a forward price of the option contract which
starts at the future time
$T'$
and expires at time
$T$,
conditional on the underlying equity index being at the level
$S_{T'}=e^{-(r(T')-d(T'))T'} F(x)$
and the whole system being in the volatility regime
$\alpha$
at time
$T'$.
The payoff function in~(\ref{eq:EuroPrice})
is completely general and can therefore depend on the
level of the underlying at
$T'$.
In order to find the value of the forward-start at time
$T'$
we must evaluate a portfolio
of 
$M(N+1)$
call options,
one for each element
$(x,\alpha)$
of the set
$\Omega\times V$,
with the corresponding strikes
$a e^{-(r(T')-d(T'))T'} F(x)$
using formula~(\ref{eq:EuroPrice}).  
The most efficient way of doing this is 
to collect all the call payoff functions into a
matrix and apply a matrix-matrix multiplication
routine 
{\tt gemm} (from LAPACK)
on the forward probability kernel (between times 
$T'$
and
$T$)
and the ``payoff matrix'' we have just created. Notice that
both of these matrices
are square and have dimension 
$M(N+1)$,
which is hence also true of the product.

Let us now define the function
$h:\Omega\times V\rightarrow \RR$
by requiring that 
$h(x,\alpha)$
equals
the diagonal element of the 
above product of matrices, which corresponds to
the index
$(x,\alpha)$.
A moment's reflection will show that
the function 
$h$
we have just defined
equals the value of the forward-start 
at time
$T'$.
In order to obtain the today's value of the forward-starting
option, all we need to do is find the current value
of the payoff
$h$
using expression~(\ref{eq:EuroPrice}).

We have therefore shown that pricing a forward-start in our
framework amounts to one matrix-matrix multiplication 
and one matrix-vector multiplication. Similarly to the
analysis of sensitivities that was carried out for European
options earlier in this subsection, we could find delta,
gamma, vega and other higher-order Greeks for the forward-starts.
However 
we are not going to pursue this any further;
given the basic ideas we have already put forth,
these algorithms would be but trivial extensions.



==> table_para.tex <==
\begin{table}
\caption{}\label{t:para}
\noindent Panel A: Parameters for the local volatilities and jumps
\begin{center}
\begin{tabular}{c c c c c c c}
$\alpha$ & $\sigma_\alpha$  & $\beta_\alpha$ & $\overline{\sigma}_\alpha$ & $\nu_\alpha^{-}$ & $\nu_\alpha^{+}$ & $\textbf{F}_\alpha$\\
\hline
0 & 0.33  & -0.50  & 0.60  & 0.41 & 0 & 50.00 \\
1 & 0.23  & -0.30  & 0.60  & 0.31 & 0 & 85.00\\
2 & 0.17  & -0.17  & 0.60  & 0.21 & 0 & 100.00\\
3 & 0.23  & 0.15  & 0.60  & 0.14 & 0 & 115.00\\
4 & 0.33  & 0.55  & 0.60  & 0.04 & 0 & 150.00\\
\end{tabular}
\end{center}




\noindent Panel B: $\G_{\alpha=1,2,3}^V$
\begin{center}
\begin{tabular}{c | c c c c c }
from/to & 0 & 1 & 2 & 3 & 4 \\
\hline
0 & -4 & 4 & 0 & 0 & 0 \\
1 & 2 & -6 & 4 & 0 & 0 \\
2 & 0 & 2 & -4 & 2 & 0 \\
3 & 0 & 0 & 4 & -6 & 2 \\
4 & 0 & 0 & 0 & 4 & -4 \\
\end{tabular}
\end{center}

\noindent Panel C: $\G_{\alpha=0}^V$
\begin{center}
\begin{tabular}{c | c c c c c }
from/to & 0 & 1 & 2 & 3 & 4 \\
\hline
0 & -4 & 4 & 0 & 0 & 0 \\
1 & 2 & -4 & 2 & 0 & 0 \\
2 & 0 & 4 & -6 & 2 & 0 \\
3 & 0 & 0 & 4 & -6 & 2 \\
4 & 0 & 0 & 0 & 4 & -4 \\
\end{tabular}
\end{center}

\noindent Panel D: $\G_{\alpha=4}^V$
\begin{center}
\begin{tabular}{c | c c c c c }
from/to & 0 & 1 & 2 & 3 & 4 \\
\hline
0 & -4 & 4 & 0 & 0 & 0 \\
1 & 2 & -6 & 4 & 0 & 0 \\
2 & 0 & 2 & -6 & 4 & 0 \\
3 & 0 & 0 & 2 & -4 & 2 \\
4 & 0 & 0 & 0 & 4 & -4 \\
\end{tabular}
\end{center}


\end{table}





==> table_result.tex <==
\begin{table}
\caption{N=75, M=1, C=16, $\sigma_0=0.2$ ,$\overline{\sigma}_0=0.6$. Closed
form represents the value of the European payoff $-{2\over (T-t)}\log({F_T\over
F_t})$, where $T-t$ is the maturity.}{}\label{t:result}
\noindent Panel A: $\nu^-=0, \nu^+=0$
\begin{center}
\begin{tabular}{c c c }
$\beta$ & closed form & lattice\\
\hline
1       & $4.000\%$  &  $4.000\%$\\
0.8     & $ 4.023\%$  &  $4.023\%$\\
0.6      & $4.060\%$  &  $4.059\%$\\
\end{tabular}
\end{center}

\noindent Panel B: $\nu^-=0.05, \nu^+=0$
\begin{center}
\begin{tabular}{c c c }
$\beta$ & closed form & lattice\\
\hline
1       & $2.896\%$  &  $2.822\%$\\
0.8     & $2.9212\%$  &  $2.844\%$\\
0.6      & $2.9547\%$  &  $2.874\%$\\
\end{tabular}
\end{center}



\end{table}





